HarmAug: Effective Data Augmentation for Knowledge Distillation of Safety Guard Models

Safety guard models that detect malicious queries aimed at large language models (LLMs) are essential for ensuring the secure and responsible deployment of LLMs in real-world applications. However, deploying existing safety guard models with billions of parameters alongside LLMs on mobile devices is impractical due to substantial memory requirements and latency. To reduce this cost, we distill a large teacher safety guard model into a smaller one using a labeled dataset of instruction-response pairs with binary harmfulness labels. Due to the limited diversity of harmful instructions in the existing labeled dataset, naively distilled models tend to underperform compared to larger models. To bridge the gap between small and large models, we propose HarmAug, a simple yet effective data augmentation method that involves jailbreaking an LLM and prompting it to generate harmful instructions. Given a prompt such as, "Make a single harmful instruction prompt that would elicit offensive content", we add an affirmative prefix (e.g., "I have an idea for a prompt:") to the LLM's response. This encourages the LLM to continue generating the rest of the response, leading to sampling harmful instructions. Another LLM generates a response to the harmful instruction, and the teacher model labels the instruction-response pair. We empirically show that our HarmAug outperforms other relevant baselines. Moreover, a 435-million-parameter safety guard model trained with HarmAug achieves an F1 score comparable to larger models with over 7 billion parameters, and even outperforms them in AUPRC, while operating at less than 25% of their computational cost.

==> figures/time_cl.tex <==
\begin{wrapfigure}{t}{0.35\textwidth}
\small
\centering
\vspace{-0.25in}
\captionof{figure}{Test F1 score on CipherChat as a function of train wallclock time.}
\vspace{-0.15in}
\includegraphics[width=\linewidth]{images/time_cipherchat_f1.pdf}
\label{fig:time}
\vspace{-0.2in}
\end{wrapfigure}

==> tables/ablation_bert_classifier.tex <==
\begin{table}[t]
\caption{Comparison with Existing BERT Safety Guard Models. We run experiments three times
with different random seeds and report the average of F1 and AUPRC scores.}
\label{tab:ablation-bert-classifier}
\resizebox{0.99\textwidth}{!}{

\begin{tabular}{lccccccccccc}
\toprule
               & & \multicolumn{2}{c}{\textbf{OAI}}                            & \multicolumn{2}{c}{\textbf{ToxicChat}}                      & \multicolumn{2}{c}{\textbf{HarmBench}}                      & \multicolumn{2}{l}{\textbf{WildGuardMix}}                    & \multicolumn{2}{c}{\textbf{Avg}} \\
\cmidrule(lr){3-4}  \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
Model          & size & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{AUPRC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{AUPRC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{AUPRC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{AUPRC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{AURPC} \\
\midrule
RoBERTa-R4 &  125M & 0.5625 & 0.6970 & 0.2217 & 0.3339 & 0.0288 & 0.6958 & 0.04778 & 0.3925 & 0.2152 & 0.5298 \\
\textbf{RoBERTa-base + Ours} & 125M 
& $0.6704$ & $0.8344$ & $0.5383$ & $0.7080$ & $0.8022$ & $0.8467$ & $0.7374$ & $0.8065$ & $0.6871$ & $0.7989$

\\
\midrule
HateBERT & 110M & 0.6442 & 0.7443 & 0.3148 & 0.4867 & 0.1423 &  0.6669 & 0.07894 & 0.3763 & 0.2951 & 0.5685
\\
\textbf{BERT-base-uncased + Ours} & 110M 
& $0.6442$ & $0.7837$ & $0.5081$ & $0.6353$ & $0.7891$ & $0.8480$ & $0.6985$ & $0.7735$ & $0.6600$ & $0.7601$

\\

\bottomrule
\end{tabular}
}
\end{table}

==> tables/ablation_data_aug_size.tex <==
\begin{table}[t]
\caption{Ablation Study on Synthetic Data Augmentation Size. We run experiments three times with different random seeds and report the average of F1 and AUPRC scores. The best results are bolded and the second-best are underlined. }
\vspace{-0.1in}
\label{tab:data-aug}
\resizebox{1.0\textwidth}{!}{

\begin{tabular}{lccccccccccc}
\toprule
               & & \multicolumn{2}{c}{\textbf{OAI}}                            & \multicolumn{2}{c}{\textbf{ToxicChat}}                      & \multicolumn{2}{c}{\textbf{HarmBench}}                      & \multicolumn{2}{l}{\textbf{WildGuardMix}}                    & \multicolumn{2}{c}{\textbf{Avg}} \\
\cmidrule(lr){3-4}  \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
Model          & size & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{AUPRC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{AUPRC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{AUPRC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{AUPRC} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{AURPC} \\
\midrule
DeBERTa & 435M 
& $0.7092$ & $0.7869$ & $0.6118$ & $0.6837$ & $0.8379$ & $0.8806$ & $0.7507$ & $0.8337$ & $0.7274$ & $0.7962$
\\
\midrule
\textbf{DeBERTa + 20K} & 435M 
& $0.7177$ & $0.8564$ & $0.6281$ & $0.7217$ & $\textbf{0.8472}$ & $0.8812$ & $0.7561$ & $\textbf{0.8409}$ & $0.7373$ & $0.8250$
\\ 
\textbf{DeBERTa + 40K} & 435M 
& $0.7192$ & $0.8558$ & $\textbf{0.6428}$ & $0.7394$ & $0.8410$ & $0.8759$ & $0.7487$ & $0.8334$ & $0.7379$ & $0.8261$
\\ 
\textbf{DeBERTa + 60K} & 435M 
& $0.7217$ & $\underline{0.8714}$ & $\underline{0.6425}$ & $\underline{0.7430}$ & $\underline{0.8421}$ & $\textbf{0.8859}$ & $0.7520$ & $0.8286$ & $\underline{0.7396}$ & $\underline{0.8322}$

\\ 
\textbf{DeBERTa + 80K} & 435M 
& $\textbf{0.7264}$ & $0.8702$ & $0.6321$ & $0.7380$ & $0.8405$ & $0.8837$ & $\textbf{0.7601}$ & $\underline{0.8356}$ & $\textbf{0.7398}$ & $0.8319$

\\ 
\textbf{DeBERTa + 100K} & 435M 
& $\underline{0.7236}$ & $\textbf{0.8791}$ & $0.6283$ & $\textbf{0.7553}$ & $0.8331$ & $\underline{0.8841}$ & $\underline{0.7576}$ & $0.8265$ & $0.7357$ & $\textbf{0.8362}$

\\ 
\bottomrule
\end{tabular}
}
\end{table}

==> tables/prefix_ablation_arxiv.tex <==
\begin{wrapfigure}{t}{0.3\textwidth}
\small
\centering
\captionof{table}{Success rate of harmful instruction generation.}
\vspace{-1em}
\resizebox{0.3\textwidth}{!}{
\begin{tabular}{lc}
\toprule
     & \textbf{Success Rate} (\%) \\
\midrule
{w/o prefix attack} & $13.02$\\
\textbf{w/ prefix attack} & $\textbf{96.81}$ \\
\bottomrule
\end{tabular}
}
\label{tab:prefix-ablation}
\vspace{-0.1in}
\end{wrapfigure}
